Leveraging Multi-lingual Positive Instances in Contrastive Learning to Improve Sentence Embedding

Learning multi-lingual sentence embeddings is a fundamental task in natural language processing. Recent trends in learning both mono-lingual and multi-lingual sentence embeddings are mainly based on contrastive learning (CL) among an anchor, one positive, and multiple negative instances. In this work, we argue that leveraging multiple positives should be considered for multi-lingual sentence embeddings because (1) positives in a diverse set of languages can benefit cross-lingual learning, and (2) transitive similarity across multiple positives can provide reliable structural information for learning. In order to investigate the impact of multiple positives in CL, we propose a novel approach, named MPCL, to effectively utilize multiple positive instances to improve the learning of multi-lingual sentence embeddings. Experimental results on various backbone models and downstream tasks demonstrate that MPCL leads to better retrieval, semantic similarity, and classification performances compared to conventional CL. We also observe that in unseen languages, sentence embedding models trained on multiple positives show better cross-lingual transfer performance than models trained on a single positive instance.

==> tables/bitext_results.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lccc}
\hline
\textbf{Model} & \textbf{BUCC} & \textbf{Tatoeba14 avg.} & \textbf{Tatoeba36 avg.} \\ \hline
INFOXLM~\cite{chi-etal-2021-infoxlm} & -   & 77.8          & 67.3 \\
LASER~\cite{artetxe2019massively} & 92.9   & 95.3          & 84.4 \\
mSimCSE$_{sw,fr}$~\cite{wang-etal-2022-english} &88.8    & 90.2         & 88.3 \\
mSimCSE$_{all}$~\cite{wang-etal-2022-english} & 95.2 & 93.2 & 91.4 \\
LaBSE~\cite{feng2020language} & 93.5   & 95.3          & 95.0 \\
\hline
mSimCSE$_{all}$~(Ours) & 95.7 & 93.2 & 91.2 \\
\ \ \ \ +Parallel & 96.1 & 93.3 & 91.2 \\
\ \ \ \ +\MN & 96.3 & 93.5 & 91.3 \\
\hline
LaBSE~(Ours) & 96.5   & 95.8          & 95.3 \\
\ \ \ \ +Parallel & 97.3   & 95.7          & 95.1 \\
\ \ \ \ +\MN & \textbf{97.7}   & \textbf{96.1}          & \textbf{95.5} \\


\hline
\end{tabular}
\caption{Results of bi-text mining tasks. We report the average score of en-xx and xx-en directions for Tatoeba and the average score of four language pairs for BUCC. model~(Ours) refers to the results we reproduced while +Parallel stands for training on parallelized dataset. \zky{results renewed}}
\label{table_main_bitext}
\end{table*}
